Stochastic and Spatial Equivalences for PALOMA

We concentrate our study on a recent process algebra - PALOMA - intended to capture interactions between spatially distributed agents, for example in collective adaptive systems. New agent-based semantic rules for deriving the underlying continuous time Markov chain are given in terms of State to Function Labelled Transition Systems. Furthermore we define a bisimulation with respect to an isometric transformation of space allowing us to compare PALOMA models with respect to their relative rather than absolute locations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{69}
\providecommand{\publicationstatus}{M.H. ter Beek and M. Loreti (Eds.): Workshop on\\ 
FORmal methods for the quantitative Evaluation\\ 
of Collective Adaptive SysTems (FORECAST'16).\\
EPTCS 217, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.217.9}{10.4204/EPTCS.217.9}}

